OT-Attack: Enhancing Adversarial Transferability of Vision-Language Models via Optimal Transport Optimization

Vision-language pre-training (VLP) models demonstrate impressive abilities in processing both images and text. However, they are vulnerable to multi-modal adversarial examples (AEs). Investigating the generation of high-transferability adversarial examples is crucial for uncovering VLP models' vulnerabilities in practical scenarios. Recent works have indicated that leveraging data augmentation and image-text modal interactions can enhance the transferability of adversarial examples for VLP models significantly. However, they do not consider the optimal alignment problem between dataaugmented image-text pairs. This oversight leads to adversarial examples that are overly tailored to the source model, thus limiting improvements in transferability. In our research, we first explore the interplay between image sets produced through data augmentation and their corresponding text sets. We find that augmented image samples can align optimally with certain texts while exhibiting less relevance to others. Motivated by this, we propose an Optimal Transport-based Adversarial Attack, dubbed OT-Attack. The proposed method formulates the features of image and text sets as two distinct distributions and employs optimal transport theory to determine the most efficient mapping between them. This optimal mapping informs our generation of adversarial examples to effectively counteract the overfitting issues. Extensive experiments across various network architectures and datasets in image-text matching tasks reveal that our OT-Attack outperforms existing state-of-the-art methods in terms of adversarial transferability.

==> table/disturbance_intensity.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\centering
\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{@{}
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c @{}}
\toprule
\cellcolor[HTML]{FFFFFF} &
  \textbf{Disturbance} &
  \cellcolor[HTML]{FFFFFF} &
  \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{ALBEF}} &
  \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{TCL}} &
  \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{CLIP\textsubscript{ViT}}} &
  \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{CLIP\textsubscript{CNN}}} \\ \cmidrule(l){4-11} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}\textbf{Source}} &
  \textbf{intensity} &
  \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}\textbf{Attack}} &
  TR R@1 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}IR R@1} &
  TR R@1 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}IR R@1} &
  TR R@1 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}IR R@1} &
  TR R@1 &
  IR R@1 \\ \midrule
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF} &
  SGA &
  \cellcolor[HTML]{EFEFEF}97.24 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}97.28} &
  45.42 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}55.25} &
  33.38 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}44.16} &
  34.93 &
  46.57 \\
\cellcolor[HTML]{FFFFFF} &
  \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}2/255} &
  Ours &
  \cellcolor[HTML]{EFEFEF}95.93 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}95.86} &
  52.37 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}61.05} &
  34.85 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}47.1} &
  42.33 &
  53.03 \\
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF} &
  SGA &
  \cellcolor[HTML]{EFEFEF}99.06 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}98.9} &
  62.17 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}68.4} &
  34.48 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}45.75} &
  42.33 &
  53.16 \\
\multirow{-4}{*}{\cellcolor[HTML]{FFFFFF}\textbf{ALBEF}} &
  \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}4/255} &
  Ours &
  \cellcolor[HTML]{EFEFEF}98.44 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}98.46} &
  72.6 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}75.33} &
  36.56 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}47.94} &
  44.05 &
  54.93 \\ \midrule
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF} &
  SGA &
  48.91 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}60.34} &
  \cellcolor[HTML]{EFEFEF}98.37 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}98.81} &
  33.87 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}44.88} &
  37.74 &
  48.3 \\
\cellcolor[HTML]{FFFFFF} &
  \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}2/255} &
  Ours &
  57.32 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}65.83} &
  \cellcolor[HTML]{EFEFEF}97.81 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}98.01} &
  34.72 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}47.16} &
  43.44 &
  54.12 \\
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF} &
  SGA &
  72.39 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}76.29} &
  \cellcolor[HTML]{EFEFEF}99.48 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}99.67} &
  35.09 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}46.07} &
  42.58 &
  54.22 \\
\multirow{-4}{*}{\cellcolor[HTML]{FFFFFF}\textbf{TCL}} &
  \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}4/255} &
  Ours &
  78.82 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}82.62} &
  \cellcolor[HTML]{EFEFEF}99.48 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}99.56} &
  39.39 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}48.87} &
  45.64 &
  56.89 \\ \midrule
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF} &
  SGA &
  13.4 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}27.22} &
  16.23 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}30.76} &
  \cellcolor[HTML]{EFEFEF}99.08 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}98.94} &
  38.76 &
  47.79 \\
\cellcolor[HTML]{FFFFFF} &
  \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}2/255} &
  Ours &
  14.29 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}29.28} &
  16.58 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}33.49} &
  \cellcolor[HTML]{EFEFEF}98.65 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}98.52} &
  43.55 &
  50.5 \\
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF} &
  SGA &
  14.08 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}29.0} &
  16.89 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}33.09} &
  \cellcolor[HTML]{EFEFEF}99.63 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}99.77} &
  46.1 &
  51.7 \\
\multirow{-4}{*}{\cellcolor[HTML]{FFFFFF}\textbf{CLIP\textsubscript{ViT}}} &
  \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}4/255} &
  Ours &
  16.79 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}31.97} &
  20.02 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}35.78} &
  \cellcolor[HTML]{EFEFEF}99.39 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}99.52} &
  49.55 &
  56.09 \\ \midrule
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF} &
  SGA &
  11.42 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}24.8} &
  14.91 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}28.82} &
  31.24 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}42.12} &
  \cellcolor[HTML]{EFEFEF}99.24 &
  \cellcolor[HTML]{EFEFEF}99.49 \\
\cellcolor[HTML]{FFFFFF} &
  \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}2/255} &
  Ours &
  11.57 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}26.24} &
  14.91 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}30.52} &
  35.63 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}48.2} &
  \cellcolor[HTML]{EFEFEF}99.39 &
  \cellcolor[HTML]{EFEFEF}99.32 \\
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF} &
  SGA &
  11.57 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}25.12} &
  16.06 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}29.75} &
  35.5 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}46.52} &
  \cellcolor[HTML]{EFEFEF}99.63 &
  \cellcolor[HTML]{EFEFEF}99.84 \\
\multirow{-4}{*}{\cellcolor[HTML]{FFFFFF}\textbf{CLIP\textsubscript{CNN}}} &
  \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}4/255} &
  Ours &
  13.14 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}26.64} &
  17.0 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}31.24} &
  37.68 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}49.78} &
  \cellcolor[HTML]{EFEFEF}99.75 &
  \cellcolor[HTML]{EFEFEF}99.65 \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Comparison of attack success rates under varying perturbation intensities. When the perturbation intensity is increased from 2/255 to 4/255, both SGA and our approach see an improved rate of attack success. Compared to the increment achieved by SGA, the enhanced transferability of our adversarial samples is more pronounced, further widening the gap in attack success rates. This indicates that our method performs more favorably under settings of stronger perturbations.}
\end{table*}
